Collu-Bench: A Benchmark for Predicting Language Model Hallucinations in Code

Despite their success, large language models (LLMs) face the critical challenge of hallucinations, generating plausible but incorrect content. While much research has focused on hallucinations in multiple modalities including images and natural language text, less attention has been given to hallucinations in source code, which leads to incorrect and vulnerable code that causes significant financial loss. To pave the way for research in LLMs' hallucinations in code, we introduce Collu-Bench, a benchmark for predicting code hallucinations of LLMs across code generation (CG) and automated program repair (APR) tasks. Collu-Bench includes 13,234 code hallucination instances collected from five datasets and 11 diverse LLMs, ranging from open-source models to commercial ones. To better understand and predict code hallucinations, Collu-Bench provides detailed features such as the per-step log probabilities of LLMs' output, token types, and the execution feedback of LLMs' generated code for in-depth analysis. In addition, we conduct experiments to predict hallucination on Collu-Bench, using both traditional machine learning techniques and neural networks, which achieves 22.03 -- 33.15% accuracy. Our experiments draw insightful findings of code hallucination patterns, reveal the challenge of accurately localizing LLMs' hallucinations, and highlight the need for more sophisticated techniques.

==> sections/ethical.tex <==
\section*{Ethical Concerns}


==> tables/bak_features.tex <==
\begin{table*}
\centering
\footnotesize
\begin{tabular}{l|l|l} 
\hline
Feature name      & Data type          & Description                                   \\ 
\hline
context\_before   & String             & The code context before the buggy line.       \\ 
\hline
context\_after    & String             & The code context after the buggy line.        \\ 
\hline
buggy\_line       & String             & The line of code that contains the bug.       \\ 
\hline
num\_steps        & Integer            & Number of tokens generated.                   \\ 
\hline
per\_step\_tokens & List[List[String]] & The top 100 tokens generated at each step.    \\ 
\hline
per\_step\_logits & List[List[Float]]  & The log probability of each token.            \\ 
\hline
tokens            & List[String]       & Generated tokens corresponding to the patch.  \\ 
\hline
types             & List[String]       & The type of each token.                       \\ 
\hline
err\_type\_before & String             & The type of error before applying the patch.  \\ 
\hline
err\_type\_after  & String             & The error message before applying the patch.  \\ 
\hline
err\_msg\_before  & String             & The type of error after applying the patch.   \\ 
\hline
err\_msg\_after   & String             & The error message after applying the patch.   \\
\hline
\end{tabular}
\caption{The names, data types, and description of the features included in the dataset.}
\label{tab: features}
\end{table*}


==> tables/bak_results.tex <==
\begin{table}
\centering
\scriptsize
\caption{Accuracy of MLP, RF, and GPT on all datasets.}
\label{tab: results}
\begin{tabular}{|l|l||c|c|c|} 
\hline
Dataset & LM  & MLP & RF & GPT \\ 
\hline
\multirow{9}{*}{Defects4J}
    & DSC-1.3b & 59.09  & 54.55  & \\ 
\cline{2-5} 
    & DSC-7b   & 40.00  & 35.00  & \\ 
\cline{2-5} 
    & SC-3b    & 100.00 & 100.00 & \\ 
\cline{2-5}
    & SC-7b    & 100.00 & 95.45  & \\ 
\cline{2-5}
    & SC-15b   & 95.45  & 90.91  & \\ 
\cline{2-5}
    & CL-7b    & 30.00  & 20.00  & \\ 
\cline{2-5}
    & CL-13b   & 27.27  & 31.82  & \\ 
\cline{2-5}
    & LMA-8b   & 36.36  & 13.64  & \\ 
\cline{2-5}
    & GPT-3.5  & 52.17  & 52.17  & \\ 
\hline
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}HumanEval-\\ Java\end{tabular}} 
    & DSC-1.3b & 66.67  & 46.67  & \\ 
\cline{2-5}
    & DSC-7b   & 13.33  & 13.33  & \\ 
\cline{2-5}
    & SC-3b    & 100.00 & 100.00 & \\ 
\cline{2-5}
    & SC-7b    & 100.00 & 100.00 & \\ 
\cline{2-5}
    & SC-15b   & 100.00 & 100.00 & \\ 
\cline{2-5}
    & CL-7b    & 40.00  & 40.00  & \\ 
\cline{2-5}
    & CL-13b   & 6.67   & 6.67   & \\ 
\cline{2-5}
    & LMA-8b   & 53.33  & 26.67  & \\ 
\cline{2-5}
    & GPT-3.5  & 26.67  & 13.33  & \\ 
\hline
\multirow{4}{*}{SWE-bench} 
    & SC-15b   & 94.79  & 94.79  & \\ 
\cline{2-5}
    & CL-13b   & 43.30  & 37.11  & \\ 
\cline{2-5}
    & LMA-8b   & 41.41  & 36.36  & \\ 
\cline{2-5}
    & GPT-3.5  & 43.88  & 41.84  & \\ 
\hline
\multirow{9}{*}{HumanEval}
    & DSC-1.3b & 53.33  & 40.00  & \\ 
\cline{2-5}
    & DSC-7b   & 46.67  & 40.00  & \\ 
\cline{2-5}
    & SC-3b    & 100.00 & 100.00 & \\ 
\cline{2-5}
    & SC-7b    & 100.00 & 100.00 & \\ 
\cline{2-5}
    & SC-15b   & 100.00 & 100.00 & \\ 
\cline{2-5}
    & CL-7b    & 60.00  & 46.67  & \\ 
\cline{2-5}
    & CL-13b   & 53.33  & 40.00  & \\ 
\cline{2-5}
    & LMA-8b   & 46.67  & 33.33  & \\ 
\cline{2-5}
    & GPT-3.5  & 73.33  & 66.67  & \\ 
\hline
\multirow{9}{*}{MBPP}
    & DSC-1.3b & 6.25   & 15.63  & \\ 
\cline{2-5}
    & DSC-7b   & 22.92  & 10.42  & \\ 
\cline{2-5}
    & SC-3b    & 21.88  & 18.75  & \\ 
\cline{2-5}
    & SC-7b    & 40.63  & 19.79  & \\ 
\cline{2-5}
    & SC-15b   & 17.71  & 20.83  & \\ 
\cline{2-5}
    & CL-7b    & 30.21  & 19.79  & \\ 
\cline{2-5}
    & CL-13b   & 16.67  & 18.75  & \\ 
\cline{2-5}
    & LMA-8b   & 1.04   & 8.33   & \\ 
\cline{2-5}
    & GPT-3.5  & 14.58  & 12.50  & \\
\hline
\end{tabular}
\end{table}

==> tables/canonical_solution_number.tex <==
\begin{table}[htp]
    \centering
    \scriptsize
    % \setlength{\tabcolsep}{5pt}
    \caption{Number of collected canonical solutions per sample in each dataset.}
    \begin{tabular}{c|ccccc}
    \toprule
         Number of Canonical Solutions & \multirow{2}{*}{HumanEval} & \multirow{2}{*}{MBPP} & \multirow{2}{*}{HumanEval-Java} & \multirow{2}{*}{Defects4J} & \multirow{2}{*}{SWE-Bench} \\
         Min. / Avg. / Max. & & & & & \\
    \midrule
         Before Program Normalization & 1 / 124.30 / 483 & 1 / 86.98 / 463 & 1 / 5.89 / 79 & 1 / 1.31 / 6 & 1 / 1.53 / 7 \\
         After Program Normalization & 1 / 82.01 / 391 & 1 / 50.01 / 319 & 1 / 5.54 / 54 & 1 / 1.31 / 6 & 1 / 1.53 / 7 \\
    \bottomrule
    \end{tabular}
    \label{tab: caconical_solution_number}
\end{table}
